Towards the D-Optimal Online Experiment Design for Recommender Selection

Selecting the optimal recommender via online exploration-exploitation is catching increasing attention where the traditional A/B testing can be slow and costly, and offline evaluations are prone to the bias of history data. Finding the optimal online experiment is nontrivial since both the users and displayed recommendations carry contextual features that are informative to the reward. While the problem can be formalized via the lens of multi-armed bandits, the existing solutions are found less satisfactorily because the general methodologies do not account for the case-specific structures, particularly for the e-commerce recommendation we study. To fill in the gap, we leverage the \emph{D-optimal design} from the classical statistics literature to achieve the maximum information gain during exploration, and reveal how it fits seamlessly with the modern infrastructure of online inference. To demonstrate the effectiveness of the optimal designs, we provide semi-synthetic simulation studies with published code and data for reproducibility purposes. We then use our deployment example on Walmart.com to fully illustrate the practical insights and effectiveness of the proposed methods.

==> notes.tex <==
One of the distinguishing features of all bandit problems studied in this book is that the learner never needs to plan for the future. More precisely, we will invariably make the assumption that the learner’s available choices and rewards tomorrow are not affected by their decisions today. Problems that do require this kind of long-term planning fall into the realm of reinforcement learning, which is the topic of the final chapter. Another limitation of the bandit framework is the assumption that the learner observes the reward in every round. The setting where the reward is not observed is called partial monitoring and is the topic of Chapter 37. Finally, often, the environment itself consists of strategic agents, which the learner needs to take into account. This problem is studied in game theory and would need a book on its own.

In traditional A/B testing the objective of the statistician is to decide which website is better. When using a bandit algorithm there is no need to end the trial. The algorithm automatically decides when one version of the site should be shown more often than another. Even if the real objective is to identify the best site, then adaptivity or early stopping can be added to the A/B process using techniques from bandit theory. While this is not the focus of this book, some of the basic ideas are explained in Chapter 33.

The learner’s goal is to maximize the total reward which is a random quantity that depends on the actions of the learner and the rewards sampled by the environment. This is not an optimization problem for three reasons:
1 What is the value of n for which we are maximizing? Occasionally prior knowledge of the horizon is reasonable, but very often the learner does not know ahead of time how many rounds are to be played.
2 The cumulative reward is a random quantity. Even if the reward distributions were known, then we require a measure of utility on distributions of Sn.
3 The learner does not know the distributions that govern the rewards for each arm.
Of these points, the last is fundamental to the bandit problem and is discussed in the next section. The lack of knowledge of the horizon is usually not a serious issue. Generally speaking it is possible to first design a policy assuming the horizon is known and then adapt it to account for the unknown horizon while proving that the loss in performance is minimal. This is almost always quite easy and there exist generic approaches for making the conversion.

For example, Langford and Zhang [2008] considers this style of policy under the name ‘epoch-greedy’ for contextual bandits (the idea of exploring then exploiting in epochs, or intervals, is essentially what Robbins [1952] suggested). We’ll return to contextual bandits in Chapter 18. Abbasi-Yadkori et al. [2009], Abbasi-Yadkori [2009b] and Rusmevichientong and Tsitsiklis [2010] consider ETC-style policies under the respective names of ‘forced exploration’ and ‘phased exploration and greedy exploitation’ (PEGE) in the context of linear bandits (which we shall meet in Chapter 19). Other names include ‘forced sampling’, ‘explore-first’, ‘explore- then-exploit’. Garivier et al. [2016b] have shown that ETC policies are necessarily suboptimal in the limit of infinite data in a way that is made precise in Chapter 16. This comment also applies to elimination based strategies, which are described in Exercise 6.8. The history of ε-greedy is unclear, but it is a popular and widely used and known algorithm in reinforcement learning [Sutton and Barto, 1998]. Auer et al. [2002a] analyze the regret of ε-greedy with slowly decreasing exploration probabilities. 

Environments that appear nonstationary can often be made stationary by adding context. For example, when bandit algorithms are used for on-line advertising, gym membership advertisements are received more positively in January than July. A bandit algorithm that is oblivious to the time of year will perceive this environment as nonstationary. You could tackle this problem by using one of the algorithms in this chapter. Or you could use a contextual bandit algorithm and include the time of year in the context. The reader is encouraged to consider whether or not adding contextual information might be preferable to using an algorithm designed for nonstationary bandits.

Nonstationary bandits have quite a long history. The celebrated Gittins index is based on a model where each arm is associated with a Markov chain that evolves when played, the reward depends on the state, and the state of the chosen Markov chain is observed after it evolves [Gittins, 1979, Gittins et al., 2011]. The classical approaches, as discussed in Chapter 35, address this problem in the Bayesian framework and the objective is primarily to design efficient algorithms rather than understanding the frequentist regret. Even more related is the restless bandit, which is the same as Gittins’ setup except the Markov chain for every arm evolves in every round, while the learner still only observes the state and reward for the action they chose. As a result, the learner needs to reason about the evolution of all the Markov chains, which makes this problem rather challenging. Restless bandits were introduced by Whittle [1988] in the Bayesian framework, where most of the results have a negative, rather than a positive character.

Contexts. In each round, an algorithm may observe some context before choosing an action. Such context often comprises the known properties of the current user, and allows for personalized actions. The algorithm has a different high-level objective. It is no longer interested in learning one good arm, since any one arm may be great for some contexts, and terrible for some others. Instead, it strives to learn the best policy which maps contexts to arms (while not spending too much time exploring).
